SN 2021foa: The "Flip-Flop" Type IIn / Ibn supernova

We present a comprehensive analysis of the photometric and spectroscopic evolution of SN~2021foa, unique among the class of transitional supernovae for repeatedly changing its spectroscopic appearance from hydrogen-to-helium-to-hydrogen-dominated (IIn-to-Ibn-to-IIn) within 50 days past peak brightness. The spectra exhibit multiple narrow ($\approx$ 300--600~km~s$^{-1}$) absorption lines of hydrogen, helium, calcium and iron together with broad helium emission lines with a full-width-at-half-maximum (FWHM) of $\sim 6000$~km~s$^{-1}$. For a steady, wind-mass loss regime, light curve modeling results in an ejecta mass of $\sim 8$ M$_{\odot}$ and CSM mass below 1 M$_{\odot}$, and an ejecta velocity consistent with the FWHM of the broad helium lines. We obtain a mass-loss rate of $\approx 2$ M$_{\odot} {\rm yr}^{-1}$. This mass-loss rate is three orders of magnitude larger than derived for normal Type II SNe. We estimate that the bulk of the CSM of SN~2021foa must have been expelled within half a year, about 15 years ago. Our analysis suggests that SN~2021foa had a helium rich ejecta which swept up a dense shell of hydrogen rich CSM shortly after explosion. At about 60 days past peak brightness, the photosphere recedes through the dense ejecta-CSM region, occulting much of the red-shifted emission of the hydrogen and helium lines, which results in observed blue-shift ($\sim -3000$~km~s$^{-1}$). Strong mass loss activity prior to explosion, such as those seen in SN~2009ip-like objects and SN~2021foa as precursor emission, are the likely origin of a complex, multiple-shell CSM close to the progenitor star.

==> table_phot.tex <==
\clearpage
\startlongtable
\begin{deluxetable*}{lcccccc}
\tablecaption{Photometry of SN2021foa}
%\tablenum{1}
\tablehead{\colhead{MJD} & \colhead{Filter} &\colhead{Magnitude} & \colhead{Error} & \colhead{System} & \colhead{Instrument} & \colhead{Telescope}} 
\startdata
59267.50 & $o$ & 19.224 & 0.291 & AB & ACAM1 & ATLAS \\
59271.50 & $o$ & 19.102 & 0.297 & AB & ACAM1 & ATLAS \\
59272.50 & $o$ & 19.351 & 0.288 & AB & ACAM1 & ATLAS \\
59277.50 & $o$ & 19.268 & 0.318 & AB & ACAM1 & ATLAS \\
59279.50 & $o$ & 19.111 & 0.190 & AB & ACAM1 & ATLAS \\
59288.50 & $o$ & 16.002 & 0.018 & AB & ACAM1 & ATLAS \\
59289.26 & $UVW1$ & 15.139 & 0.050 & Vega & UVOT & Swift \\
59289.27 & $U$ & 14.820 & 0.043 & Vega & UVOT & Swift \\
59289.27 & $B$ & 15.916 & 0.060 & Vega & UVOT & Swift \\
59289.29 & $UVW2$ & 15.957 & 0.061 & Vega & UVOT & Swift \\
59289.29 & $V$ & 15.678 & 0.086 & Vega & UVOT & Swift \\
59289.33 & $U$ & 15.573 & 0.078 & Vega & UVOT & Swift \\
59290.79 & $U$ & 15.356 & 0.049 & Vega & UVOT & Swift \\
59290.79 & $UVW2$ & 15.790 & 0.049 & Vega & UVOT & Swift \\
59290.79 & $V$ & 15.419 & 0.078 & Vega & UVOT & Swift \\
59290.79 & $U$ & 14.605 & 0.043 & Vega & UVOT & Swift \\
59290.80 & $B$ & 15.759 & 0.067 & Vega & UVOT & Swift \\
59290.80 & $UVW1$ & 14.958 & 0.048 & Vega & UVOT & Swift \\
59290.87 & $gp$ & 15.558 & 0.016 & AB & Sinistro & LCO \\
59290.87 & $rp$ & 15.649 & 0.017 & AB & Sinistro & LCO \\
59290.87 & $ip$ & 15.803 & 0.021 & AB & Sinistro & LCO \\
59291.52 & $B$ & 15.591 & 0.019 & AB & Sinistro & LCO \\
59291.52 & $V$ & 15.343 & 0.015 & AB & Sinistro & LCO \\
59291.52 & $R$ & 15.394 & 0.014 & AB & Sinistro & LCO \\
59291.64 & $UVW2$ & 15.715 & 0.054 & Vega & UVOT & Swift \\
59291.65 & $U$ & 15.316 & 0.054 & Vega & UVOT & Swift \\
59291.65 & $V$ & 15.220 & 0.085 & Vega & UVOT & Swift \\
59291.65 & $U$ & 14.439 & 0.045 & Vega & UVOT & Swift \\
59291.65 & $B$ & 15.667 & 0.079 & Vega & UVOT & Swift \\
59291.65 & $UVW1$ & 14.837 & 0.051 & Vega & UVOT & Swift \\
59292.39 & $B$ & 15.439 & 0.017 & AB & Sinistro & LCO \\
59292.39 & $B$ & 15.449 & 0.017 & AB & Sinistro & LCO \\
59292.39 & $V$ & 15.379 & 0.016 & AB & Sinistro & LCO \\
59292.39 & $V$ & 15.382 & 0.017 & AB & Sinistro & LCO \\
59292.39 & $gp$ & 15.429 & 0.014 & AB & Sinistro & LCO \\
59292.39 & $gp$ & 15.349 & 0.013 & AB & Sinistro & LCO \\
59292.39 & $rp$ & 15.474 & 0.015 & AB & Sinistro & LCO \\
59292.39 & $rp$ & 15.430 & 0.015 & AB & Sinistro & LCO \\
59292.40 & $ip$ & 15.553 & 0.018 & AB & Sinistro & LCO \\
59292.40 & $ip$ & 15.570 & 0.018 & AB & Sinistro & LCO \\
59292.50 & $o$ & 15.488 & 0.010 & AB & ACAM1 & ATLAS \\
59292.71 & $V$ & 15.398 & 0.076 & Vega & UVOT & Swift \\
59292.72 & $U$ & 14.326 & 0.040 & Vega & UVOT & Swift \\
59292.84 & $U$ & 15.272 & 0.048 & Vega & UVOT & Swift \\
59292.84 & $UVW2$ & 15.688 & 0.047 & Vega & UVOT & Swift \\
59292.85 & $UVW1$ & 14.839 & 0.046 & Vega & UVOT & Swift \\
59292.85 & $B$ & 15.935 & 0.062 & Vega & UVOT & Swift \\
59292.87 & $B$ & 15.435 & 0.018 & AB & Sinistro & LCO \\
59292.87 & $V$ & 15.243 & 0.018 & AB & Sinistro & LCO \\
59292.87 & $R$ & 15.271 & 0.015 & AB & Sinistro & LCO \\
59292.87 & $I$ & 15.163 & 0.029 & AB & Sinistro & LCO \\
59293.50 & $c$ & 15.390 & 0.009 & AB & ACAM1 & ATLAS \\
59294.26 & $z$ & 15.489 & 0.084 & AB & - & Thacher \\
59294.26 & $i$ & 15.401 & 0.039 & AB & - & Thacher \\
59294.26 & $r$ & 15.263 & 0.021 & AB & - & Thacher \\
59294.27 & $g$ & 15.320 & 0.022 & AB & - & Thacher \\
59294.90 & $B$ & 15.282 & 0.016 & AB & Sinistro & LCO \\
59294.90 & $V$ & 15.214 & 0.016 & AB & Sinistro & LCO \\
59294.90 & $R$ & 15.147 & 0.014 & AB & Sinistro & LCO \\
59294.90 & $I$ & 14.947 & 0.018 & AB & Sinistro & LCO \\
59295.25 & $r$ & 14.991 & 0.022 & AB & - & Thacher \\
59295.25 & $g$ & 15.143 & 0.043 & AB & - & Thacher \\
59295.35 & $U$ & 15.531 & 0.020 & AB & Sinistro & LCO \\
59295.35 & $U$ & 15.535 & 0.024 & AB & Sinistro & LCO \\
59295.35 & $B$ & 15.293 & 0.016 & AB & Sinistro & LCO \\
59295.36 & $B$ & 15.301 & 0.016 & AB & Sinistro & LCO \\
59295.36 & $V$ & 15.197 & 0.015 & AB & Sinistro & LCO \\
59295.36 & $V$ & 15.202 & 0.015 & AB & Sinistro & LCO \\
59295.36 & $gp$ & 15.209 & 0.013 & AB & Sinistro & LCO \\
59295.36 & $gp$ & 15.208 & 0.013 & AB & Sinistro & LCO \\
59295.36 & $rp$ & 15.293 & 0.014 & AB & Sinistro & LCO \\
59295.36 & $rp$ & 15.280 & 0.014 & AB & Sinistro & LCO \\
59295.36 & $ip$ & 15.364 & 0.016 & AB & Sinistro & LCO \\
59295.36 & $ip$ & 15.287 & 0.017 & AB & Sinistro & LCO \\
59295.45 & $V$ & 15.322 & 0.059 & AB & Nickel & Lick \\
59295.46 & $V$ & 15.198 & 0.085 & AB & Nickel & Lick \\
59295.46 & $r$ & 15.294 & 0.027 & AB & Nickel & Lick \\
59295.46 & $i$ & 15.416 & 0.043 & AB & Nickel & Lick \\
59295.50 & $o$ & 15.337 & 0.009 & AB & ACAM1 & ATLAS \\
59295.80 & $up$ & 15.482 & 0.030 & AB & Sinistro & LCO \\
59295.81 & $gp$ & 15.305 & 0.016 & AB & Sinistro & LCO \\
59295.81 & $rp$ & 15.185 & 0.016 & AB & Sinistro & LCO \\
59295.81 & $ip$ & 15.272 & 0.021 & AB & Sinistro & LCO \\
59296.26 & $i$ & 14.994 & 0.098 & AB & - & Thacher \\
59296.26 & $r$ & 15.029 & 0.020 & AB & - & Thacher \\
59296.27 & $g$ & 15.134 & 0.034 & AB & - & Thacher \\
59297.44 & $z$ & 15.063 & 0.020 & AB & - & Thacher \\
59297.45 & $i$ & 14.990 & 0.024 & AB & - & Thacher \\
59297.45 & $r$ & 15.031 & 0.020 & AB & - & Thacher \\
59297.45 & $g$ & 15.162 & 0.025 & AB & - & Thacher \\
59298.34 & $B$ & 15.130 & 0.015 & AB & Sinistro & LCO \\
59298.34 & $B$ & 15.182 & 0.014 & AB & Sinistro & LCO \\
59298.34 & $V$ & 15.075 & 0.015 & AB & Sinistro & LCO \\
59298.34 & $V$ & 15.074 & 0.015 & AB & Sinistro & LCO \\
59298.48 & $U$ & 15.280 & 0.020 & AB & Sinistro & LCO \\
59298.48 & $U$ & 15.259 & 0.019 & AB & Sinistro & LCO \\
59298.48 & $B$ & 15.281 & 0.015 & AB & Sinistro & LCO \\
59298.48 & $B$ & 15.270 & 0.015 & AB & Sinistro & LCO \\
59298.49 & $V$ & 15.051 & 0.015 & AB & Sinistro & LCO \\
59298.49 & $V$ & 15.062 & 0.015 & AB & Sinistro & LCO \\
59298.49 & $gp$ & 15.157 & 0.013 & AB & Sinistro & LCO \\
59298.49 & $gp$ & 15.171 & 0.013 & AB & Sinistro & LCO \\
59298.49 & $rp$ & 15.154 & 0.016 & AB & Sinistro & LCO \\
59298.49 & $rp$ & 15.113 & 0.016 & AB & Sinistro & LCO \\
59298.49 & $ip$ & 15.258 & 0.022 & AB & Sinistro & LCO \\
59298.49 & $ip$ & 15.258 & 0.020 & AB & Sinistro & LCO \\
59298.81 & $B$ & 15.189 & 0.016 & AB & Sinistro & LCO \\
59298.81 & $V$ & 15.045 & 0.015 & AB & Sinistro & LCO \\
59298.82 & $R$ & 14.968 & 0.014 & AB & Sinistro & LCO \\
59298.82 & $I$ & 14.820 & 0.018 & AB & Sinistro & LCO \\
59299.26 & $z$ & 15.185 & 0.100 & AB & - & Thacher \\
59299.26 & $i$ & 15.189 & 0.100 & AB & - & Thacher \\
59299.50 & $o$ & 15.149 & 0.009 & AB & ACAM1 & ATLAS \\
59300.25 & $z$ & 14.869 & 0.100 & AB & - & Thacher \\
59300.25 & $i$ & 14.927 & 0.100 & AB & - & Thacher \\
59300.26 & $r$ & 14.659 & 0.100 & AB & - & Thacher \\
59300.26 & $g$ & 15.012 & 0.100 & AB & - & Thacher \\
59300.50 & $o$ & 15.173 & 0.016 & AB & ACAM1 & ATLAS \\
59300.78 & $U$ & 16.210 & 0.066 & Vega & UVOT & Swift \\
59300.78 & $UVW2$ & 16.268 & 0.055 & Vega & UVOT & Swift \\
59300.78 & $B$ & 15.392 & 0.050 & Vega & UVOT & Swift \\
59300.78 & $V$ & 15.113 & 0.062 & Vega & UVOT & Swift \\
59300.78 & $U$ & 14.401 & 0.041 & Vega & UVOT & Swift \\
59300.78 & $UVW1$ & 15.414 & 0.052 & Vega & UVOT & Swift \\
59300.80 & $up$ & 15.343 & 0.024 & AB & Sinistro & LCO \\
59300.80 & $gp$ & 15.111 & 0.019 & AB & Sinistro & LCO \\
59300.81 & $rp$ & 15.136 & 0.019 & AB & Sinistro & LCO \\
59300.81 & $ip$ & 15.264 & 0.023 & AB & Sinistro & LCO \\
59301.04 & $B$ & 15.275 & 0.017 & AB & Sinistro & LCO \\
59301.05 & $V$ & 15.049 & 0.016 & AB & Sinistro & LCO \\
59301.05 & $R$ & 14.913 & 0.016 & AB & Sinistro & LCO \\
59301.05 & $I$ & 14.750 & 0.020 & AB & Sinistro & LCO \\
59301.24 & $z$ & 15.243 & 0.100 & AB & - & Thacher \\
59301.24 & $i$ & 15.182 & 0.100 & AB & - & Thacher \\
59301.25 & $r$ & 15.088 & 0.100 & AB & - & Thacher \\
59301.25 & $g$ & 15.172 & 0.100 & AB & - & Thacher \\
59301.31 & $U$ & 15.388 & 0.024 & AB & Sinistro & LCO \\
59301.31 & $B$ & 15.221 & 0.017 & AB & Sinistro & LCO \\
59301.31 & $B$ & 15.288 & 0.018 & AB & Sinistro & LCO \\
59301.31 & $V$ & 15.032 & 0.017 & AB & Sinistro & LCO \\
59301.31 & $V$ & 15.031 & 0.018 & AB & Sinistro & LCO \\
59301.31 & $gp$ & 15.081 & 0.016 & AB & Sinistro & LCO \\
59301.32 & $gp$ & 15.098 & 0.016 & AB & Sinistro & LCO \\
59301.38 & $V$ & 15.088 & 0.056 & Vega & UVOT & Swift \\
59301.38 & $UVW2$ & 16.364 & 0.052 & Vega & UVOT & Swift \\
59301.38 & $B$ & 15.423 & 0.048 & Vega & UVOT & Swift \\
59301.38 & $U$ & 14.471 & 0.040 & Vega & UVOT & Swift \\
59301.38 & $UVW1$ & 15.414 & 0.049 & Vega & UVOT & Swift \\
59301.38 & $U$ & 16.297 & 0.066 & Vega & UVOT & Swift \\
59302.23 & $z$ & 14.743 & 0.100 & AB & - & Thacher \\
59302.23 & $i$ & 14.934 & 0.100 & AB & - & Thacher \\
59302.23 & $r$ & 14.935 & 0.100 & AB & - & Thacher \\
59302.24 & $g$ & 14.953 & 0.100 & AB & - & Thacher \\
59303.22 & $z$ & 15.284 & 0.100 & AB & - & Thacher \\
59303.22 & $i$ & 15.197 & 0.100 & AB & - & Thacher \\
59303.22 & $r$ & 15.089 & 0.100 & AB & - & Thacher \\
59303.22 & $g$ & 15.103 & 0.100 & AB & - & Thacher \\
59304.79 & $B$ & 15.303 & 0.016 & AB & Sinistro & LCO \\
59304.79 & $V$ & 15.148 & 0.015 & AB & Sinistro & LCO \\
59304.79 & $R$ & 15.009 & 0.014 & AB & Sinistro & LCO \\
59304.79 & $I$ & 14.735 & 0.017 & AB & Sinistro & LCO \\
59304.84 & $U$ & 15.558 & 0.021 & AB & Sinistro & LCO \\
59304.84 & $U$ & 15.588 & 0.021 & AB & Sinistro & LCO \\
59304.84 & $B$ & 15.301 & 0.016 & AB & Sinistro & LCO \\
59304.84 & $B$ & 15.299 & 0.016 & AB & Sinistro & LCO \\
59304.84 & $V$ & 15.110 & 0.017 & AB & Sinistro & LCO \\
59304.84 & $V$ & 15.131 & 0.017 & AB & Sinistro & LCO \\
59304.85 & $gp$ & 15.153 & 0.015 & AB & Sinistro & LCO \\
59304.85 & $gp$ & 15.120 & 0.015 & AB & Sinistro & LCO \\
59304.85 & $rp$ & 15.122 & 0.017 & AB & Sinistro & LCO \\
59304.85 & $rp$ & 15.110 & 0.020 & AB & Sinistro & LCO \\
59304.85 & $ip$ & 15.201 & 0.024 & AB & Sinistro & LCO \\
59304.85 & $ip$ & 15.193 & 0.024 & AB & Sinistro & LCO \\
59305.23 & $z$ & 15.220 & 0.046 & AB & - & Thacher \\
59305.23 & $i$ & 15.135 & 0.020 & AB & - & Thacher \\
59305.23 & $r$ & 15.089 & 0.020 & AB & - & Thacher \\
59305.23 & $g$ & 15.219 & 0.020 & AB & - & Thacher \\
59305.50 & $o$ & 15.187 & 0.009 & AB & ACAM1 & ATLAS \\
59306.03 & $up$ & 15.647 & 0.018 & AB & Sinistro & LCO \\
59306.04 & $gp$ & 15.321 & 0.015 & AB & Sinistro & LCO \\
59306.04 & $rp$ & 15.217 & 0.015 & AB & Sinistro & LCO \\
59306.04 & $ip$ & 15.247 & 0.020 & AB & Sinistro & LCO \\
59306.22 & $z$ & 15.162 & 0.053 & AB & - & Thacher \\
59306.23 & $i$ & 15.190 & 0.026 & AB & - & Thacher \\
59306.23 & $r$ & 15.102 & 0.025 & AB & - & Thacher \\
59306.23 & $g$ & 15.241 & 0.020 & AB & - & Thacher \\
59306.43 & $V$ & 15.409 & 0.009 & AB & Nickel & Lick \\
59306.43 & $V$ & 15.172 & 0.103 & AB & Nickel & Lick \\
59306.43 & $r$ & 15.212 & 0.038 & AB & Nickel & Lick \\
59306.44 & $i$ & 15.263 & 0.052 & AB & Nickel & Lick \\
59307.22 & $z$ & 15.392 & 0.057 & AB & - & Thacher \\
59307.22 & $i$ & 15.222 & 0.059 & AB & - & Thacher \\
59307.22 & $r$ & 15.165 & 0.020 & AB & - & Thacher \\
59307.22 & $g$ & 15.269 & 0.028 & AB & - & Thacher \\
59307.69 & $B$ & 15.473 & 0.015 & AB & Sinistro & LCO \\
59307.69 & $V$ & 15.229 & 0.014 & AB & Sinistro & LCO \\
59307.69 & $R$ & 15.081 & 0.013 & AB & Sinistro & LCO \\
59307.69 & $I$ & 14.786 & 0.015 & AB & Sinistro & LCO \\
59307.74 & $U$ & 15.751 & 0.022 & AB & Sinistro & LCO \\
59307.74 & $U$ & 15.779 & 0.024 & AB & Sinistro & LCO \\
59307.74 & $B$ & 15.496 & 0.016 & AB & Sinistro & LCO \\
59307.74 & $B$ & 15.488 & 0.016 & AB & Sinistro & LCO \\
59307.75 & $V$ & 15.239 & 0.016 & AB & Sinistro & LCO \\
59307.75 & $V$ & 15.256 & 0.016 & AB & Sinistro & LCO \\
59307.75 & $gp$ & 15.296 & 0.013 & AB & Sinistro & LCO \\
59307.75 & $gp$ & 15.317 & 0.013 & AB & Sinistro & LCO \\
59307.75 & $rp$ & 15.251 & 0.014 & AB & Sinistro & LCO \\
59307.75 & $rp$ & 15.239 & 0.014 & AB & Sinistro & LCO \\
59307.75 & $ip$ & 15.281 & 0.017 & AB & Sinistro & LCO \\
59307.75 & $ip$ & 15.275 & 0.017 & AB & Sinistro & LCO \\
59308.23 & $z$ & 15.290 & 0.020 & AB & - & Thacher \\
59308.23 & $i$ & 15.273 & 0.021 & AB & - & Thacher \\
59308.23 & $r$ & 15.222 & 0.020 & AB & - & Thacher \\
59308.23 & $g$ & 15.321 & 0.020 & AB & - & Thacher \\
59309.41 & $V$ & 15.564 & 0.041 & AB & Nickel & Lick \\
59309.41 & $V$ & 15.279 & 0.035 & AB & Nickel & Lick \\
59309.41 & $r$ & 15.315 & 0.038 & AB & Nickel & Lick \\
59309.42 & $i$ & 15.336 & 0.036 & AB & Nickel & Lick \\
59310.07 & $V$ & 15.461 & 0.024 & AB & Sinistro & LCO \\
59310.07 & $gp$ & 15.518 & 0.015 & AB & Sinistro & LCO \\
59310.07 & $rp$ & 15.368 & 0.017 & AB & Sinistro & LCO \\
59310.16 & $B$ & 15.707 & 0.029 & AB & Sinistro & LCO \\
59310.16 & $V$ & 15.517 & 0.020 & AB & Sinistro & LCO \\
59310.16 & $R$ & 15.184 & 0.021 & AB & Sinistro & LCO \\
59310.16 & $I$ & 14.971 & 0.031 & AB & Sinistro & LCO \\
59311.27 & $z$ & 15.346 & 0.023 & AB & - & Thacher \\
59311.27 & $i$ & 15.264 & 0.024 & AB & - & Thacher \\
59311.27 & $r$ & 15.316 & 0.020 & AB & - & Thacher \\
59311.27 & $g$ & 15.474 & 0.020 & AB & - & Thacher \\
59311.50 & $c$ & 15.516 & 0.008 & AB & ACAM1 & ATLAS \\
59311.78 & $B$ & 15.780 & 0.019 & AB & Sinistro & LCO \\
59311.78 & $V$ & 15.517 & 0.016 & AB & Sinistro & LCO \\
59311.78 & $R$ & 15.252 & 0.014 & AB & Sinistro & LCO \\
59311.78 & $I$ & 14.917 & 0.016 & AB & Sinistro & LCO \\
59312.24 & $z$ & 15.237 & 0.035 & AB & - & Thacher \\
59312.24 & $i$ & 15.174 & 0.036 & AB & - & Thacher \\
59312.24 & $r$ & 15.234 & 0.021 & AB & - & Thacher \\
59312.24 & $g$ & 15.474 & 0.030 & AB & - & Thacher \\
59312.88 & $B$ & 15.811 & 0.017 & AB & Sinistro & LCO \\
59312.88 & $B$ & 15.800 & 0.016 & AB & Sinistro & LCO \\
59312.88 & $V$ & 15.555 & 0.017 & AB & Sinistro & LCO \\
59312.88 & $V$ & 15.549 & 0.017 & AB & Sinistro & LCO \\
59312.89 & $gp$ & 15.638 & 0.014 & AB & Sinistro & LCO \\
59312.89 & $gp$ & 15.659 & 0.014 & AB & Sinistro & LCO \\
59312.89 & $rp$ & 15.486 & 0.015 & AB & Sinistro & LCO \\
59312.89 & $rp$ & 15.493 & 0.014 & AB & Sinistro & LCO \\
59312.89 & $ip$ & 15.492 & 0.016 & AB & Sinistro & LCO \\
59312.89 & $ip$ & 15.479 & 0.017 & AB & Sinistro & LCO \\
59313.28 & $z$ & 15.356 & 0.028 & AB & - & Thacher \\
59313.28 & $i$ & 15.315 & 0.024 & AB & - & Thacher \\
59313.28 & $r$ & 15.390 & 0.020 & AB & - & Thacher \\
59313.89 & $UVW1$ & 17.211 & 0.167 & Vega & UVOT & Swift \\
59313.89 & $U$ & 15.807 & 0.078 & Vega & UVOT & Swift \\
59313.89 & $B$ & 16.159 & 0.094 & Vega & UVOT & Swift \\
59313.89 & $V$ & 15.812 & 0.124 & Vega & UVOT & Swift \\
59313.89 & $U$ & 18.109 & 0.302 & Vega & UVOT & Swift \\
59314.23 & $g$ & 15.589 & 0.020 & AB & - & Thacher \\
59314.44 & $B$ & 16.097 & 0.021 & AB & Sinistro & LCO \\
59314.44 & $V$ & 15.761 & 0.018 & AB & Sinistro & LCO \\
59314.44 & $R$ & 15.359 & 0.014 & AB & Sinistro & LCO \\
59314.44 & $I$ & 15.164 & 0.019 & AB & Sinistro & LCO \\
59315.40 & $up$ & 16.600 & 0.022 & AB & Sinistro & LCO \\
59315.40 & $gp$ & 15.657 & 0.016 & AB & Sinistro & LCO \\
59315.40 & $rp$ & 15.594 & 0.016 & AB & Sinistro & LCO \\
59315.40 & $ip$ & 15.721 & 0.019 & AB & Sinistro & LCO \\
59315.45 & $B$ & 16.119 & 0.020 & AB & Sinistro & LCO \\
59315.45 & $V$ & 15.855 & 0.018 & AB & Sinistro & LCO \\
59315.45 & $R$ & 15.418 & 0.015 & AB & Sinistro & LCO \\
59315.45 & $I$ & 15.224 & 0.020 & AB & Sinistro & LCO \\
59315.74 & $U$ & 16.068 & 0.135 & Vega & UVOT & Swift \\
59315.74 & $V$ & 15.862 & 0.127 & Vega & UVOT & Swift \\
59316.51 & $B$ & 16.142 & 0.018 & AB & Sinistro & LCO \\
59316.51 & $B$ & 16.147 & 0.018 & AB & Sinistro & LCO \\
59316.51 & $V$ & 15.793 & 0.017 & AB & Sinistro & LCO \\
59316.52 & $V$ & 15.791 & 0.018 & AB & Sinistro & LCO \\
59316.52 & $gp$ & 15.732 & 0.014 & AB & Sinistro & LCO \\
59316.52 & $gp$ & 15.722 & 0.014 & AB & Sinistro & LCO \\
59316.52 & $rp$ & 15.735 & 0.015 & AB & Sinistro & LCO \\
59316.52 & $rp$ & 15.771 & 0.015 & AB & Sinistro & LCO \\
59316.52 & $ip$ & 15.749 & 0.019 & AB & Sinistro & LCO \\
59316.52 & $ip$ & 15.788 & 0.018 & AB & Sinistro & LCO \\
59317.13 & $V$ & 15.888 & 0.022 & AB & Sinistro & LCO \\
59317.13 & $R$ & 15.576 & 0.017 & AB & Sinistro & LCO \\
59317.13 & $I$ & 15.237 & 0.023 & AB & Sinistro & LCO \\
59317.18 & $i$ & 15.599 & 0.021 & AB & - & Thacher \\
59318.40 & $V$ & 15.860 & 0.126 & AB & Nickel & Lick \\
59318.40 & $i$ & 15.963 & 0.055 & AB & Nickel & Lick \\
59319.23 & $i$ & 15.437 & 0.020 & AB & - & Thacher \\
59319.23 & $r$ & 15.496 & 0.020 & AB & - & Thacher \\
59319.23 & $g$ & 15.696 & 0.031 & AB & - & Thacher \\
59319.50 & $c$ & 15.832 & 0.008 & AB & ACAM1 & ATLAS \\
59319.78 & $B$ & 16.101 & 0.020 & AB & Sinistro & LCO \\
59319.78 & $B$ & 16.100 & 0.021 & AB & Sinistro & LCO \\
59319.78 & $V$ & 15.847 & 0.020 & AB & Sinistro & LCO \\
59319.78 & $V$ & 15.875 & 0.020 & AB & Sinistro & LCO \\
59319.79 & $gp$ & 15.809 & 0.015 & AB & Sinistro & LCO \\
59319.79 & $gp$ & 15.828 & 0.015 & AB & Sinistro & LCO \\
59319.79 & $rp$ & 15.705 & 0.016 & AB & Sinistro & LCO \\
59319.79 & $rp$ & 15.789 & 0.016 & AB & Sinistro & LCO \\
59319.79 & $ip$ & 15.811 & 0.020 & AB & Sinistro & LCO \\
59319.79 & $ip$ & 15.803 & 0.021 & AB & Sinistro & LCO \\
59319.80 & $V$ & 15.855 & 0.020 & AB & Sinistro & LCO \\
59319.80 & $R$ & 15.623 & 0.021 & AB & Sinistro & LCO \\
59319.80 & $I$ & 15.284 & 0.026 & AB & Sinistro & LCO \\
59320.18 & $z$ & 15.601 & 0.041 & AB & - & Thacher \\
59320.18 & $i$ & 15.536 & 0.020 & AB & - & Thacher \\
59320.18 & $r$ & 15.610 & 0.027 & AB & - & Thacher \\
59320.18 & $g$ & 15.833 & 0.030 & AB & - & Thacher \\
59321.18 & $z$ & 15.559 & 0.056 & AB & - & Thacher \\
59321.18 & $i$ & 15.686 & 0.030 & AB & - & Thacher \\
59321.18 & $r$ & 15.602 & 0.031 & AB & - & Thacher \\
59321.19 & $g$ & 15.796 & 0.038 & AB & - & Thacher \\
59321.39 & $gp$ & 15.889 & 0.017 & AB & Sinistro & LCO \\
59321.40 & $rp$ & 15.748 & 0.016 & AB & Sinistro & LCO \\
59321.40 & $ip$ & 15.855 & 0.019 & AB & Sinistro & LCO \\
59321.50 & $o$ & 15.707 & 0.012 & AB & ACAM1 & ATLAS \\
59321.62 & $V$ & 15.881 & 0.020 & AB & Sinistro & LCO \\
59321.62 & $R$ & 15.652 & 0.018 & AB & Sinistro & LCO \\
59321.62 & $I$ & 15.297 & 0.023 & AB & Sinistro & LCO \\
59322.18 & $g$ & 15.647 & 0.033 & AB & - & Thacher \\
59322.18 & $r$ & 15.401 & 0.023 & AB & - & Thacher \\
59322.18 & $i$ & 15.383 & 0.036 & AB & - & Thacher \\
59322.19 & $z$ & 15.447 & 0.022 & AB & - & Thacher \\
59323.19 & $g$ & 15.789 & 0.031 & AB & - & Thacher \\
59323.19 & $r$ & 15.504 & 0.020 & AB & - & Thacher \\
59323.50 & $o$ & 15.796 & 0.013 & AB & ACAM1 & ATLAS \\
59324.19 & $g$ & 15.945 & 0.020 & AB & - & Thacher \\
59324.19 & $r$ & 15.779 & 0.020 & AB & - & Thacher \\
59324.33 & $V$ & 16.311 & 0.033 & AB & Nickel & Lick \\
59324.33 & $V$ & 15.897 & 0.094 & AB & Nickel & Lick \\
59324.34 & $r$ & 15.893 & 0.061 & AB & Nickel & Lick \\
59324.34 & $i$ & 15.890 & 0.042 & AB & Nickel & Lick \\
59324.50 & $o$ & 15.865 & 0.014 & AB & ACAM1 & ATLAS \\
59324.89 & $U$ & 17.008 & 0.030 & AB & Sinistro & LCO \\
59324.89 & $U$ & 16.927 & 0.031 & AB & Sinistro & LCO \\
59324.89 & $B$ & 16.295 & 0.018 & AB & Sinistro & LCO \\
59324.89 & $B$ & 16.252 & 0.018 & AB & Sinistro & LCO \\
59324.89 & $V$ & 15.924 & 0.017 & AB & Sinistro & LCO \\
59324.89 & $V$ & 15.918 & 0.017 & AB & Sinistro & LCO \\
59324.89 & $gp$ & 16.041 & 0.015 & AB & Sinistro & LCO \\
59324.90 & $gp$ & 16.038 & 0.015 & AB & Sinistro & LCO \\
59324.90 & $rp$ & 15.881 & 0.015 & AB & Sinistro & LCO \\
59324.90 & $rp$ & 15.899 & 0.016 & AB & Sinistro & LCO \\
59324.90 & $ip$ & 15.819 & 0.054 & AB & Sinistro & LCO \\
59324.90 & $ip$ & 15.827 & 0.058 & AB & Sinistro & LCO \\
59325.21 & $g$ & 16.079 & 0.020 & AB & - & Thacher \\
59325.21 & $r$ & 15.870 & 0.020 & AB & - & Thacher \\
59325.21 & $i$ & 15.817 & 0.020 & AB & - & Thacher \\
59325.21 & $z$ & 15.838 & 0.020 & AB & - & Thacher \\
59325.76 & $B$ & 16.353 & 0.045 & AB & Sinistro & LCO \\
59325.76 & $V$ & 16.070 & 0.042 & AB & Sinistro & LCO \\
59325.76 & $R$ & 15.703 & 0.027 & AB & Sinistro & LCO \\
59325.77 & $I$ & 15.503 & 0.037 & AB & Sinistro & LCO \\
59326.54 & $up$ & 17.282 & 0.023 & AB & Sinistro & LCO \\
59326.54 & $gp$ & 16.089 & 0.018 & AB & Sinistro & LCO \\
59326.54 & $rp$ & 16.024 & 0.017 & AB & Sinistro & LCO \\
59326.54 & $ip$ & 15.995 & 0.065 & AB & Sinistro & LCO \\
59327.01 & $B$ & 16.471 & 0.034 & AB & Sinistro & LCO \\
59327.01 & $V$ & 16.077 & 0.028 & AB & Sinistro & LCO \\
59327.01 & $R$ & 15.775 & 0.023 & AB & Sinistro & LCO \\
59327.01 & $I$ & 15.544 & 0.028 & AB & Sinistro & LCO \\
59327.50 & $o$ & 16.062 & 0.018 & AB & ACAM1 & ATLAS \\
59328.50 & $o$ & 16.169 & 0.021 & AB & ACAM1 & ATLAS \\
59329.19 & $g$ & 16.450 & 0.038 & AB & - & Thacher \\
59329.20 & $r$ & 16.148 & 0.041 & AB & - & Thacher \\
59329.20 & $i$ & 16.170 & 0.024 & AB & - & Thacher \\
59329.20 & $z$ & 16.216 & 0.028 & AB & - & Thacher \\
59332.20 & $g$ & 16.588 & 0.027 & AB & - & Thacher \\
59332.20 & $r$ & 16.276 & 0.020 & AB & - & Thacher \\
59332.20 & $i$ & 16.181 & 0.025 & AB & - & Thacher \\
59332.20 & $z$ & 16.166 & 0.025 & AB & - & Thacher \\
59332.47 & $U$ & 17.846 & 0.078 & AB & Sinistro & LCO \\
59332.47 & $U$ & 18.007 & 0.085 & AB & Sinistro & LCO \\
59332.48 & $B$ & 17.283 & 0.037 & AB & Sinistro & LCO \\
59332.48 & $B$ & 17.285 & 0.036 & AB & Sinistro & LCO \\
59332.48 & $V$ & 16.766 & 0.029 & AB & Sinistro & LCO \\
59332.48 & $V$ & 16.802 & 0.032 & AB & Sinistro & LCO \\
59332.48 & $gp$ & 16.923 & 0.024 & AB & Sinistro & LCO \\
59332.48 & $gp$ & 16.940 & 0.027 & AB & Sinistro & LCO \\
59332.48 & $rp$ & 16.678 & 0.029 & AB & Sinistro & LCO \\
59332.48 & $rp$ & 16.693 & 0.029 & AB & Sinistro & LCO \\
59332.50 & $o$ & 16.727 & 0.035 & AB & ACAM1 & ATLAS \\
59332.87 & $B$ & 17.263 & 0.068 & AB & Sinistro & LCO \\
59332.87 & $V$ & 16.866 & 0.072 & AB & Sinistro & LCO \\
59332.87 & $R$ & 16.458 & 0.082 & AB & Sinistro & LCO \\
59332.87 & $I$ & 16.098 & 0.213 & AB & Sinistro & LCO \\
59333.50 & $o$ & 16.774 & 0.026 & AB & ACAM1 & ATLAS \\
59334.50 & $o$ & 16.877 & 0.026 & AB & ACAM1 & ATLAS \\
59335.20 & $g$ & 17.222 & 0.020 & AB & - & Thacher \\
59335.20 & $r$ & 16.902 & 0.020 & AB & - & Thacher \\
59335.20 & $i$ & 16.912 & 0.020 & AB & - & Thacher \\
59335.21 & $z$ & 16.753 & 0.020 & AB & - & Thacher \\
59335.50 & $o$ & 17.004 & 0.040 & AB & ACAM1 & ATLAS \\
59335.87 & $up$ & 18.649 & 0.043 & AB & Sinistro & LCO \\
59335.87 & $gp$ & 17.329 & 0.027 & AB & Sinistro & LCO \\
59335.88 & $rp$ & 16.988 & 0.023 & AB & Sinistro & LCO \\
59335.88 & $ip$ & 16.950 & 0.068 & AB & Sinistro & LCO \\
59335.91 & $B$ & 17.735 & 0.038 & AB & Sinistro & LCO \\
59335.91 & $V$ & 17.170 & 0.027 & AB & Sinistro & LCO \\
59335.91 & $R$ & 16.785 & 0.021 & AB & Sinistro & LCO \\
59335.91 & $I$ & 16.445 & 0.028 & AB & Sinistro & LCO \\
59336.31 & $V$ & 17.950 & 0.104 & AB & Nickel & Lick \\
59336.32 & $V$ & 17.459 & 0.094 & AB & Nickel & Lick \\
59336.32 & $r$ & 17.300 & 0.060 & AB & Nickel & Lick \\
59336.32 & $i$ & 17.029 & 0.069 & AB & Nickel & Lick \\
59337.38 & $V$ & 17.302 & 0.052 & AB & Sinistro & LCO \\
59337.39 & $R$ & 16.851 & 0.032 & AB & Sinistro & LCO \\
59337.39 & $I$ & 16.575 & 0.040 & AB & Sinistro & LCO \\
59337.48 & $B$ & 17.820 & 0.030 & AB & Sinistro & LCO \\
59337.48 & $B$ & 17.760 & 0.030 & AB & Sinistro & LCO \\
59337.48 & $V$ & 17.135 & 0.025 & AB & Sinistro & LCO \\
59337.48 & $V$ & 17.202 & 0.027 & AB & Sinistro & LCO \\
59337.48 & $gp$ & 17.426 & 0.020 & AB & Sinistro & LCO \\
59337.49 & $gp$ & 17.492 & 0.020 & AB & Sinistro & LCO \\
59337.49 & $rp$ & 17.104 & 0.021 & AB & Sinistro & LCO \\
59337.49 & $rp$ & 17.088 & 0.022 & AB & Sinistro & LCO \\
59337.49 & $ip$ & 17.020 & 0.087 & AB & Sinistro & LCO \\
59337.49 & $ip$ & 17.145 & 0.081 & AB & Sinistro & LCO \\
59337.50 & $c$ & 17.339 & 0.024 & AB & ACAM1 & ATLAS \\
59338.21 & $z$ & 16.784 & 0.069 & AB & - & Thacher \\
59339.20 & $g$ & 17.355 & 0.020 & AB & - & Thacher \\
59339.20 & $r$ & 16.953 & 0.020 & AB & - & Thacher \\
59339.21 & $i$ & 16.779 & 0.021 & AB & - & Thacher \\
59339.21 & $z$ & 16.756 & 0.020 & AB & - & Thacher \\
59339.33 & $V$ & 17.914 & 0.064 & AB & Nickel & Lick \\
59339.34 & $V$ & 17.240 & 0.074 & AB & Nickel & Lick \\
59339.34 & $r$ & 17.164 & 0.036 & AB & Nickel & Lick \\
59339.34 & $i$ & 17.141 & 0.043 & AB & Nickel & Lick \\
59340.19 & $B$ & 18.015 & 0.062 & AB & Sinistro & LCO \\
59340.19 & $B$ & 17.994 & 0.065 & AB & Sinistro & LCO \\
59340.20 & $V$ & 17.245 & 0.038 & AB & Sinistro & LCO \\
59340.20 & $B$ & 18.033 & 0.057 & AB & Sinistro & LCO \\
59340.20 & $B$ & 18.020 & 0.065 & AB & Sinistro & LCO \\
59340.20 & $V$ & 17.325 & 0.037 & AB & Sinistro & LCO \\
59340.21 & $V$ & 17.356 & 0.035 & AB & Sinistro & LCO \\
59340.21 & $gp$ & 17.563 & 0.023 & AB & Sinistro & LCO \\
59340.21 & $gp$ & 17.540 & 0.023 & AB & Sinistro & LCO \\
59340.21 & $rp$ & 17.131 & 0.023 & AB & Sinistro & LCO \\
59340.21 & $rp$ & 17.159 & 0.024 & AB & Sinistro & LCO \\
59340.21 & $ip$ & 17.029 & 0.082 & AB & Sinistro & LCO \\
59340.21 & $ip$ & 17.062 & 0.091 & AB & Sinistro & LCO \\
59340.30 & $g$ & 17.303 & 0.020 & AB & - & Thacher \\
59340.31 & $r$ & 16.885 & 0.020 & AB & - & Thacher \\
59340.31 & $i$ & 16.801 & 0.020 & AB & - & Thacher \\
59340.31 & $z$ & 16.652 & 0.021 & AB & - & Thacher \\
59342.11 & $B$ & 17.929 & 0.041 & AB & Sinistro & LCO \\
59342.11 & $B$ & 17.930 & 0.041 & AB & Sinistro & LCO \\
59342.11 & $V$ & 17.429 & 0.034 & AB & Sinistro & LCO \\
59342.11 & $V$ & 17.373 & 0.030 & AB & Sinistro & LCO \\
59342.11 & $gp$ & 17.667 & 0.023 & AB & Sinistro & LCO \\
59342.11 & $gp$ & 17.664 & 0.023 & AB & Sinistro & LCO \\
59342.11 & $rp$ & 17.271 & 0.024 & AB & Sinistro & LCO \\
59342.12 & $rp$ & 17.289 & 0.023 & AB & Sinistro & LCO \\
59342.12 & $ip$ & 17.327 & 0.100 & AB & Sinistro & LCO \\
59342.12 & $ip$ & 17.262 & 0.087 & AB & Sinistro & LCO \\
59343.99 & $B$ & 18.081 & 0.033 & AB & Sinistro & LCO \\
59343.99 & $B$ & 18.102 & 0.033 & AB & Sinistro & LCO \\
59343.99 & $V$ & 17.492 & 0.030 & AB & Sinistro & LCO \\
59343.99 & $V$ & 17.548 & 0.030 & AB & Sinistro & LCO \\
59343.99 & $gp$ & 17.770 & 0.024 & AB & Sinistro & LCO \\
59344.00 & $gp$ & 17.771 & 0.024 & AB & Sinistro & LCO \\
59344.00 & $rp$ & 17.357 & 0.024 & AB & Sinistro & LCO \\
59344.00 & $rp$ & 17.310 & 0.024 & AB & Sinistro & LCO \\
59344.00 & $ip$ & 17.247 & 0.080 & AB & Sinistro & LCO \\
59344.00 & $ip$ & 17.288 & 0.089 & AB & Sinistro & LCO \\
59344.50 & $o$ & 17.406 & 0.063 & AB & ACAM1 & ATLAS \\
59345.16 & $B$ & 18.385 & 0.066 & AB & Sinistro & LCO \\
59345.16 & $B$ & 18.358 & 0.062 & AB & Sinistro & LCO \\
59345.16 & $V$ & 17.722 & 0.041 & AB & Sinistro & LCO \\
59345.16 & $V$ & 17.699 & 0.037 & AB & Sinistro & LCO \\
59345.16 & $gp$ & 17.937 & 0.026 & AB & Sinistro & LCO \\
59345.17 & $gp$ & 17.975 & 0.027 & AB & Sinistro & LCO \\
59345.17 & $rp$ & 17.512 & 0.027 & AB & Sinistro & LCO \\
59345.17 & $rp$ & 17.477 & 0.026 & AB & Sinistro & LCO \\
59345.17 & $ip$ & 17.318 & 0.082 & AB & Sinistro & LCO \\
59345.17 & $ip$ & 17.337 & 0.091 & AB & Sinistro & LCO \\
59346.23 & $g$ & 17.831 & 0.020 & AB & - & Thacher \\
59346.23 & $r$ & 17.332 & 0.020 & AB & - & Thacher \\
59346.24 & $i$ & 17.243 & 0.020 & AB & - & Thacher \\
59346.24 & $z$ & 17.151 & 0.020 & AB & - & Thacher \\
59347.24 & $B$ & 18.330 & 0.087 & AB & Sinistro & LCO \\
59347.24 & $B$ & 18.550 & 0.259 & AB & Sinistro & LCO \\
59347.40 & $U$ & 19.320 & 0.183 & AB & Sinistro & LCO \\
59347.41 & $B$ & 18.607 & 0.060 & AB & Sinistro & LCO \\
59347.41 & $B$ & 18.673 & 0.099 & AB & Sinistro & LCO \\
59347.41 & $V$ & 17.805 & 0.297 & AB & Sinistro & LCO \\
59347.41 & $V$ & 17.620 & 0.290 & AB & Sinistro & LCO \\
59347.41 & $gp$ & 18.251 & 0.080 & AB & Sinistro & LCO \\
59347.41 & $gp$ & 18.352 & 0.106 & AB & Sinistro & LCO \\
59347.41 & $rp$ & 17.835 & 0.066 & AB & Sinistro & LCO \\
59347.42 & $rp$ & 17.864 & 0.075 & AB & Sinistro & LCO \\
59347.42 & $ip$ & 17.718 & 0.118 & AB & Sinistro & LCO \\
59347.42 & $ip$ & 17.702 & 0.084 & AB & Sinistro & LCO \\
59348.25 & $g$ & 17.726 & 0.029 & AB & - & Thacher \\
59348.26 & $r$ & 17.494 & 0.020 & AB & - & Thacher \\
59348.26 & $i$ & 17.262 & 0.113 & AB & - & Thacher \\
59348.28 & $z$ & 17.177 & 0.027 & AB & - & Thacher \\
59348.32 & $V$ & 18.673 & 0.065 & AB & Nickel & Lick \\
59348.32 & $V$ & 17.980 & 0.087 & AB & Nickel & Lick \\
59348.33 & $r$ & 17.792 & 0.047 & AB & Nickel & Lick \\
59348.33 & $i$ & 17.769 & 0.049 & AB & Nickel & Lick \\
59348.50 & $o$ & 17.748 & 0.075 & AB & ACAM1 & ATLAS \\
59349.07 & $B$ & 18.909 & 0.084 & AB & Sinistro & LCO \\
59349.07 & $B$ & 18.972 & 0.091 & AB & Sinistro & LCO \\
59349.07 & $V$ & 17.996 & 0.054 & AB & Sinistro & LCO \\
59349.07 & $V$ & 18.027 & 0.053 & AB & Sinistro & LCO \\
59349.07 & $gp$ & 18.362 & 0.033 & AB & Sinistro & LCO \\
59349.07 & $gp$ & 18.364 & 0.035 & AB & Sinistro & LCO \\
59349.07 & $rp$ & 17.797 & 0.029 & AB & Sinistro & LCO \\
59349.07 & $rp$ & 17.676 & 0.032 & AB & Sinistro & LCO \\
59349.08 & $ip$ & 17.866 & 0.067 & AB & Sinistro & LCO \\
59349.08 & $ip$ & 17.730 & 0.093 & AB & Sinistro & LCO \\
59349.09 & $B$ & 18.958 & 0.033 & AB & Sinistro & LCO \\
59349.10 & $V$ & 18.011 & 0.028 & AB & Sinistro & LCO \\
59349.10 & $R$ & 17.681 & 0.026 & AB & Sinistro & LCO \\
59349.10 & $I$ & 17.209 & 0.037 & AB & Sinistro & LCO \\
59349.50 & $c$ & 18.256 & 0.074 & AB & ACAM1 & ATLAS \\
59350.91 & $B$ & 19.005 & 0.114 & AB & Sinistro & LCO \\
59350.91 & $B$ & 19.005 & 0.143 & AB & Sinistro & LCO \\
59350.91 & $V$ & 18.553 & 0.092 & AB & Sinistro & LCO \\
59350.91 & $V$ & 18.481 & 0.085 & AB & Sinistro & LCO \\
59350.91 & $gp$ & 18.469 & 0.038 & AB & Sinistro & LCO \\
59350.91 & $gp$ & 18.444 & 0.039 & AB & Sinistro & LCO \\
59350.91 & $rp$ & 17.958 & 0.036 & AB & Sinistro & LCO \\
59350.92 & $rp$ & 17.933 & 0.034 & AB & Sinistro & LCO \\
59350.92 & $ip$ & 17.971 & 0.081 & AB & Sinistro & LCO \\
59350.92 & $ip$ & 18.040 & 0.077 & AB & Sinistro & LCO \\
59351.28 & $V$ & 18.960 & 0.067 & AB & Nickel & Lick \\
59351.29 & $V$ & 18.429 & 0.090 & AB & Nickel & Lick \\
59351.29 & $r$ & 18.147 & 0.060 & AB & Nickel & Lick \\
59351.30 & $i$ & 18.420 & 0.080 & AB & Nickel & Lick \\
59351.50 & $o$ & 17.944 & 0.092 & AB & ACAM1 & ATLAS \\
59351.74 & $B$ & 18.746 & 0.059 & AB & Sinistro & LCO \\
59351.74 & $V$ & 18.481 & 0.046 & AB & Sinistro & LCO \\
59351.74 & $R$ & 17.762 & 0.025 & AB & Sinistro & LCO \\
59351.74 & $I$ & 17.304 & 0.040 & AB & Sinistro & LCO \\
59352.61 & $B$ & 18.972 & 0.061 & AB & Sinistro & LCO \\
59352.61 & $B$ & 18.997 & 0.063 & AB & Sinistro & LCO \\
59352.61 & $V$ & 18.455 & 0.050 & AB & Sinistro & LCO \\
59352.62 & $V$ & 18.456 & 0.053 & AB & Sinistro & LCO \\
59352.62 & $gp$ & 18.567 & 0.029 & AB & Sinistro & LCO \\
59352.62 & $gp$ & 18.595 & 0.033 & AB & Sinistro & LCO \\
59352.62 & $rp$ & 18.121 & 0.029 & AB & Sinistro & LCO \\
59352.62 & $rp$ & 18.104 & 0.030 & AB & Sinistro & LCO \\
59352.62 & $ip$ & 18.167 & 0.108 & AB & Sinistro & LCO \\
59352.62 & $ip$ & 18.005 & 0.100 & AB & Sinistro & LCO \\
59353.50 & $o$ & 18.137 & 0.110 & AB & ACAM1 & ATLAS \\
59353.97 & $B$ & 19.362 & 0.209 & AB & Sinistro & LCO \\
59353.97 & $V$ & 18.719 & 0.111 & AB & Sinistro & LCO \\
59353.97 & $gp$ & 18.698 & 0.051 & AB & Sinistro & LCO \\
59353.97 & $gp$ & 18.638 & 0.050 & AB & Sinistro & LCO \\
59353.97 & $rp$ & 18.177 & 0.048 & AB & Sinistro & LCO \\
59353.98 & $rp$ & 18.212 & 0.055 & AB & Sinistro & LCO \\
59353.98 & $ip$ & 18.214 & 0.127 & AB & Sinistro & LCO \\
59354.40 & $U$ & 19.802 & 0.268 & AB & Sinistro & LCO \\
59354.40 & $U$ & 19.453 & 0.169 & AB & Sinistro & LCO \\
59354.41 & $B$ & 19.137 & 0.074 & AB & Sinistro & LCO \\
59354.41 & $B$ & 18.967 & 0.065 & AB & Sinistro & LCO \\
59354.41 & $V$ & 18.741 & 0.048 & AB & Sinistro & LCO \\
59354.41 & $V$ & 18.746 & 0.049 & AB & Sinistro & LCO \\
59354.41 & $gp$ & 18.662 & 0.038 & AB & Sinistro & LCO \\
59354.41 & $gp$ & 18.679 & 0.037 & AB & Sinistro & LCO \\
59354.41 & $rp$ & 18.208 & 0.036 & AB & Sinistro & LCO \\
59354.41 & $rp$ & 18.271 & 0.038 & AB & Sinistro & LCO \\
59354.42 & $ip$ & 18.029 & 0.149 & AB & Sinistro & LCO \\
59354.42 & $ip$ & 17.998 & 0.152 & AB & Sinistro & LCO \\
59355.50 & $o$ & 17.948 & 0.128 & AB & ACAM1 & ATLAS \\
59356.32 & $V$ & 19.389 & 0.173 & AB & Nickel & Lick \\
59356.32 & $V$ & 18.724 & 0.103 & AB & Nickel & Lick \\
59356.33 & $r$ & 18.411 & 0.083 & AB & Nickel & Lick \\
59356.33 & $i$ & 18.309 & 0.074 & AB & Nickel & Lick \\
59358.90 & $B$ & 19.096 & 0.229 & AB & Sinistro & LCO \\
59358.90 & $V$ & 18.769 & 0.214 & AB & Sinistro & LCO \\
59358.91 & $R$ & 18.075 & 0.106 & AB & Sinistro & LCO \\
59358.91 & $I$ & 17.650 & 0.106 & AB & Sinistro & LCO \\
59359.20 & $V$ & 19.422 & 0.143 & AB & Nickel & Lick \\
59359.20 & $V$ & 18.827 & 0.118 & AB & Nickel & Lick \\
59359.21 & $r$ & 18.486 & 0.067 & AB & Nickel & Lick \\
59359.21 & $i$ & 18.404 & 0.071 & AB & Nickel & Lick \\
59360.08 & $U$ & 19.622 & 0.220 & AB & Sinistro & LCO \\
59360.08 & $U$ & 19.569 & 0.201 & AB & Sinistro & LCO \\
59360.08 & $B$ & 19.296 & 0.133 & AB & Sinistro & LCO \\
59360.08 & $B$ & 19.433 & 0.145 & AB & Sinistro & LCO \\
59360.09 & $V$ & 18.839 & 0.135 & AB & Sinistro & LCO \\
59360.09 & $V$ & 18.894 & 0.140 & AB & Sinistro & LCO \\
59360.09 & $gp$ & 18.993 & 0.100 & AB & Sinistro & LCO \\
59360.09 & $gp$ & 19.094 & 0.112 & AB & Sinistro & LCO \\
59360.09 & $rp$ & 18.471 & 0.093 & AB & Sinistro & LCO \\
59360.09 & $rp$ & 18.577 & 0.097 & AB & Sinistro & LCO \\
59360.09 & $ip$ & 18.375 & 0.192 & AB & Sinistro & LCO \\
59360.09 & $ip$ & 18.400 & 0.101 & AB & Sinistro & LCO \\
59360.50 & $o$ & 18.590 & 0.214 & AB & ACAM1 & ATLAS \\
59362.21 & $V$ & 19.942 & 0.173 & AB & Nickel & Lick \\
59362.21 & $V$ & 18.411 & 0.103 & AB & Nickel & Lick \\
59362.22 & $r$ & 18.463 & 0.065 & AB & Nickel & Lick \\
59362.22 & $i$ & 17.899 & 0.081 & AB & Nickel & Lick \\
59362.50 & $o$ & 18.978 & 0.269 & AB & ACAM1 & ATLAS \\
59363.51 & $gp$ & 19.230 & 0.071 & AB & Sinistro & LCO \\
59363.51 & $rp$ & 18.831 & 0.048 & AB & Sinistro & LCO \\
59363.51 & $ip$ & 18.537 & 0.151 & AB & Sinistro & LCO \\
59364.70 & $B$ & 19.572 & 0.169 & AB & Sinistro & LCO \\
59364.70 & $B$ & 19.590 & 0.216 & AB & Sinistro & LCO \\
59364.70 & $V$ & 18.976 & 0.193 & AB & Sinistro & LCO \\
59364.70 & $V$ & 18.983 & 0.197 & AB & Sinistro & LCO \\
59364.70 & $gp$ & 19.327 & 0.064 & AB & Sinistro & LCO \\
59364.70 & $gp$ & 19.273 & 0.066 & AB & Sinistro & LCO \\
59364.71 & $rp$ & 18.707 & 0.084 & AB & Sinistro & LCO \\
59364.71 & $rp$ & 18.966 & 0.079 & AB & Sinistro & LCO \\
59364.71 & $ip$ & 19.068 & 0.190 & AB & Sinistro & LCO \\
59364.71 & $ip$ & 19.097 & 0.146 & AB & Sinistro & LCO \\
59364.75 & $B$ & 19.621 & 0.124 & AB & Sinistro & LCO \\
59364.76 & $V$ & 18.988 & 0.078 & AB & Sinistro & LCO \\
59364.76 & $R$ & 18.694 & 0.029 & AB & Sinistro & LCO \\
59364.77 & $I$ & 18.106 & 0.059 & AB & Sinistro & LCO \\
59366.50 & $o$ & 19.189 & 0.294 & AB & ACAM1 & ATLAS \\
59367.19 & $B$ & 19.858 & 0.144 & AB & Sinistro & LCO \\
59367.19 & $V$ & 19.081 & 0.036 & AB & Sinistro & LCO \\
59367.20 & $R$ & 18.868 & 0.030 & AB & Sinistro & LCO \\
59367.20 & $I$ & 18.197 & 0.035 & AB & Sinistro & LCO \\
59367.50 & $c$ & 19.247 & 0.173 & AB & ACAM1 & ATLAS \\
59371.50 & $c$ & 19.655 & 0.250 & AB & ACAM1 & ATLAS \\
59371.70 & $U$ & 19.714 & 0.269 & AB & Sinistro & LCO \\
59371.70 & $B$ & 19.872 & 0.145 & AB & Sinistro & LCO \\
59371.70 & $B$ & 19.928 & 0.110 & AB & Sinistro & LCO \\
59371.70 & $V$ & 19.150 & 0.093 & AB & Sinistro & LCO \\
59371.71 & $V$ & 19.136 & 0.124 & AB & Sinistro & LCO \\
59371.71 & $gp$ & 19.649 & 0.086 & AB & Sinistro & LCO \\
59371.71 & $rp$ & 19.401 & 0.095 & AB & Sinistro & LCO \\
59373.50 & $o$ & 19.153 & 0.276 & AB & ACAM1 & ATLAS \\
59376.98 & $B$ & 20.086 & 0.242 & AB & Sinistro & LCO \\
59376.98 & $V$ & 19.214 & 0.139 & AB & Sinistro & LCO \\
59376.99 & $R$ & 19.275 & 0.048 & AB & Sinistro & LCO \\
59376.99 & $I$ & 18.486 & 0.096 & AB & Sinistro & LCO \\
59377.50 & $o$ & 19.364 & 0.335 & AB & ACAM1 & ATLAS \\
59379.12 & $up$ & 20.849 & 0.119 & AB & Sinistro & LCO \\
59379.13 & $gp$ & 19.879 & 0.092 & AB & Sinistro & LCO \\
59379.13 & $rp$ & 19.632 & 0.110 & AB & Sinistro & LCO \\
59379.13 & $ip$ & 19.184 & 0.115 & AB & Sinistro & LCO \\
59379.50 & $c$ & 19.489 & 0.216 & AB & ACAM1 & ATLAS \\
59383.83 & $rp$ & 19.614 & 0.187 & AB & Sinistro & LCO \\
59383.83 & $ip$ & 19.686 & 0.297 & AB & Sinistro & LCO \\
59386.08 & $rp$ & 19.405 & 0.181 & AB & Sinistro & LCO \\
59387.10 & $B$ & 20.121 & 0.250 & AB & Sinistro & LCO \\
59387.10 & $B$ & 20.113 & 0.229 & AB & Sinistro & LCO \\
59387.11 & $gp$ & 20.053 & 0.300 & AB & Sinistro & LCO \\
59387.11 & $gp$ & 20.107 & 0.306 & AB & Sinistro & LCO \\
59387.11 & $rp$ & 19.308 & 0.156 & AB & Sinistro & LCO \\
59389.90 & $rp$ & 19.229 & 0.290 & AB & Sinistro & LCO \\
59392.45 & $gp$ & 19.631 & 0.145 & AB & Sinistro & LCO \\
59392.45 & $gp$ & 19.687 & 0.139 & AB & Sinistro & LCO \\
59392.45 & $gp$ & 19.647 & 0.115 & AB & Sinistro & LCO \\
59392.45 & $rp$ & 19.220 & 0.170 & AB & Sinistro & LCO \\
59392.45 & $rp$ & 19.257 & 0.168 & AB & Sinistro & LCO \\
59392.46 & $z$ & 17.877 & 0.249 & AB & Sinistro & LCO \\
59392.46 & $z$ & 17.487 & 0.219 & AB & Sinistro & LCO \\
59393.10 & $up$ & 20.997 & 0.276 & AB & Sinistro & LCO \\
59393.10 & $gp$ & 19.908 & 0.204 & AB & Sinistro & LCO \\
59393.11 & $rp$ & 19.325 & 0.187 & AB & Sinistro & LCO \\
59395.16 & $rp$ & 19.369 & 0.221 & AB & Sinistro & LCO \\
59397.44 & $up$ & 21.432 & 0.198 & AB & Sinistro & LCO \\
59397.45 & $gp$ & 19.895 & 0.186 & AB & Sinistro & LCO \\
59397.45 & $rp$ & 19.462 & 0.171 & AB & Sinistro & LCO \\
59398.01 & $B$ & 20.556 & 0.263 & AB & Sinistro & LCO \\
59398.01 & $B$ & 20.321 & 0.135 & AB & Sinistro & LCO \\
59398.01 & $V$ & 19.725 & 0.114 & AB & Sinistro & LCO \\
59398.01 & $V$ & 19.829 & 0.119 & AB & Sinistro & LCO \\
59398.02 & $gp$ & 19.968 & 0.168 & AB & Sinistro & LCO \\
59398.02 & $gp$ & 19.847 & 0.185 & AB & Sinistro & LCO \\
59398.02 & $rp$ & 19.573 & 0.145 & AB & Sinistro & LCO \\
59398.02 & $rp$ & 19.535 & 0.147 & AB & Sinistro & LCO \\
59398.03 & $ip$ & 19.809 & 0.296 & AB & Sinistro & LCO \\
59398.03 & $ip$ & 19.746 & 0.289 & AB & Sinistro & LCO \\
59399.48 & $gp$ & 20.175 & 0.150 & AB & Sinistro & LCO \\
59399.48 & $rp$ & 19.505 & 0.185 & AB & Sinistro & LCO \\
59399.48 & $ip$ & 19.395 & 0.188 & AB & Sinistro & LCO \\
59400.86 & $gp$ & 20.340 & 0.233 & AB & Sinistro & LCO \\
59400.86 & $rp$ & 19.466 & 0.140 & AB & Sinistro & LCO \\
59401.38 & $gp$ & 20.012 & 0.255 & AB & Sinistro & LCO \\
59401.38 & $gp$ & 20.155 & 0.251 & AB & Sinistro & LCO \\
59401.38 & $gp$ & 20.174 & 0.254 & AB & Sinistro & LCO \\
59401.39 & $rp$ & 19.433 & 0.145 & AB & Sinistro & LCO \\
59401.39 & $rp$ & 19.469 & 0.144 & AB & Sinistro & LCO \\
59401.39 & $z$ & 18.444 & 0.083 & AB & Sinistro & LCO \\
59401.39 & $z$ & 18.449 & 0.101 & AB & Sinistro & LCO \\
59406.52 & $gp$ & 20.479 & 0.235 & AB & Sinistro & LCO \\
59406.52 & $rp$ & 19.505 & 0.166 & AB & Sinistro & LCO \\
59406.52 & $ip$ & 19.450 & 0.326 & AB & Sinistro & LCO \\
59409.06 & $B$ & 20.483 & 0.148 & AB & Sinistro & LCO \\
59409.06 & $B$ & 20.252 & 0.140 & AB & Sinistro & LCO \\
59409.06 & $V$ & 20.104 & 0.256 & AB & Sinistro & LCO \\
59409.06 & $V$ & 20.104 & 0.257 & AB & Sinistro & LCO \\
59409.06 & $gp$ & 20.405 & 0.253 & AB & Sinistro & LCO \\
59409.07 & $gp$ & 20.442 & 0.256 & AB & Sinistro & LCO \\
59409.07 & $rp$ & 19.343 & 0.153 & AB & Sinistro & LCO \\
59409.07 & $rp$ & 19.288 & 0.151 & AB & Sinistro & LCO \\
59409.50 & $c$ & 19.686 & 0.274 & AB & ACAM1 & ATLAS \\
59411.50 & $o$ & 19.031 & 0.255 & AB & ACAM1 & ATLAS \\
59420.35 & $B$ & 20.548 & 0.204 & AB & Sinistro & LCO \\
59420.35 & $B$ & 20.586 & 0.232 & AB & Sinistro & LCO \\
59420.36 & $V$ & 20.266 & 0.188 & AB & Sinistro & LCO \\
59420.36 & $V$ & 20.207 & 0.196 & AB & Sinistro & LCO \\
59420.36 & $gp$ & 20.401 & 0.279 & AB & Sinistro & LCO \\
59420.36 & $gp$ & 20.423 & 0.288 & AB & Sinistro & LCO \\
59420.37 & $rp$ & 19.819 & 0.159 & AB & Sinistro & LCO \\
59420.37 & $rp$ & 19.803 & 0.175 & AB & Sinistro & LCO \\
59425.38 & $gp$ & 20.547 & 0.261 & AB & Sinistro & LCO \\
59425.38 & $gp$ & 20.545 & 0.261 & AB & Sinistro & LCO \\
59425.39 & $rp$ & 19.898 & 0.244 & AB & Sinistro & LCO \\
59425.39 & $z$ & 19.120 & 0.081 & AB & Sinistro & LCO \\
59425.39 & $z$ & 19.138 & 0.105 & AB & Sinistro & LCO \\
59425.42 & $gp$ & 20.529 & 0.200 & AB & Sinistro & LCO \\
59425.42 & $rp$ & 19.864 & 0.257 & AB & Sinistro & LCO \\
59427.81 & $rp$ & 19.941 & 0.195 & AB & Sinistro & LCO \\
59432.77 & $gp$ & 20.483 & 0.208 & AB & Sinistro & LCO \\
59432.77 & $rp$ & 19.955 & 0.221 & AB & Sinistro & LCO \\
59432.97 & $V$ & 20.436 & 0.309 & AB & Sinistro & LCO \\
59432.98 & $V$ & 20.439 & 0.265 & AB & Sinistro & LCO \\
59432.98 & $gp$ & 20.630 & 0.170 & AB & Sinistro & LCO \\
59432.98 & $gp$ & 20.846 & 0.218 & AB & Sinistro & LCO \\
59432.98 & $rp$ & 19.911 & 0.234 & AB & Sinistro & LCO \\
59432.99 & $rp$ & 20.034 & 0.223 & AB & Sinistro & LCO \\
59438.04 & $gp$ & 20.902 & 0.230 & AB & Sinistro & LCO \\
59438.04 & $rp$ & 20.038 & 0.239 & AB & Sinistro & LCO \\
59443.38 & $gp$ & 20.311 & 0.285 & AB & Sinistro & LCO \\
59443.38 & $rp$ & 20.112 & 0.225 & AB & Sinistro & LCO \\
59449.99 & $gp$ & 20.425 & 0.278 & AB & Sinistro & LCO \\
59450.00 & $gp$ & 20.457 & 0.254 & AB & Sinistro & LCO \\
59450.00 & $rp$ & 20.156 & 0.231 & AB & Sinistro & LCO \\
59450.00 & $rp$ & 20.259 & 0.275 & AB & Sinistro & LCO \\
59451.74 & $rp$ & 20.250 & 0.260 & AB & Sinistro & LCO \\
\enddata
\end{deluxetable*}
